Localization-Based Beam Focusing in Near-Field Communications

Shifting 6G-and-beyond wireless systems to higher frequency bands and the utilization of massive multiple-input multiple-output arrays will extend the near-field region, affecting beamforming and user localization schemes. In this paper, we propose a localization-based beam-focusing design, in which the receive combiners are directly constructed from the steering vectors corresponding to the estimated user locations. To support this approach, we analyze the 2D-MUSIC algorithm by examining its spectrum in simplified, tractable setups with minimal numbers of antennas and users. Lastly, we compare the proposed localization-based beam focusing, with locations estimated via 2D-MUSIC, with pilot-based zero forcing in terms of uplink sum spectral efficiency. Our results show significant gains under dominant line-of-sight propagation, short coherence blocks, and high noise power typical of high-frequency systems.

==> figures/Error_SD_N128.tex <==
2.41935000 0.04630000 0.05075357
2.64976429 nan 0.06094491
2.88017857 nan 0.07214180
3.11059286 nan 0.08428061
3.34100714 nan 0.09729770
3.57142143 nan 0.11112940
3.80183571 nan 0.12571210
4.03225000 0.12480000 0.14098214
4.32026786 nan 0.16146717
4.60828571 nan 0.18381951
4.89630357 nan 0.20785683
5.18432143 nan 0.23339684
5.47233929 nan 0.26025720
5.76035714 nan 0.28825563
6.04837500 0.29080000 0.31720981
6.33639286 nan 0.34747560
6.62441071 nan 0.37949352
6.91242857 nan 0.41320824
7.20044643 nan 0.44856443
7.48846429 nan 0.48550677
7.77648214 nan 0.52397992
8.06450000 0.50850000 0.56392855
8.64053571 nan 0.64793607
9.21657143 nan 0.73735017
9.79260714 nan 0.83226570
10.36864286 nan 0.93277753
10.94467857 nan 1.03898049
11.52071429 nan 1.15096944
12.09675000 1.18930000 1.26883923

==> figures/Error_SD_N64.tex <==
0.59535000 0.01110000 0.01174620
0.65205000 nan 0.01410484
0.70875000 nan 0.01669620
0.76545000 nan 0.01950556
0.82215000 nan 0.02251817
0.87885000 nan 0.02571933
0.93555000 nan 0.02909429
0.99225000 0.03120000 0.03262832
1.06312500 nan 0.03736929
1.13400000 nan 0.04254242
1.20487500 nan 0.04810552
1.27575000 nan 0.05401639
1.34662500 nan 0.06023285
1.41750000 nan 0.06671269
1.48837500 0.06960000 0.07341372
1.55925000 nan 0.08041831
1.63012500 nan 0.08782840
1.70100000 nan 0.09563120
1.77187500 nan 0.10381389
1.84275000 nan 0.11236367
1.91362500 nan 0.12126774
1.98450000 0.12530000 0.13051328
2.12625000 nan 0.14995563
2.26800000 nan 0.17064926
2.40975000 nan 0.19261612
2.55150000 nan 0.21587816
2.69325000 nan 0.24045733
2.83500000 nan 0.26637559
2.97675000 0.28500000 0.29365488

==> figures/Error_var_N128.tex <==
2.41e+00 2.14e-03 2.57e-03
2.64e+00 nan 3.71e-03
2.88e+00 nan 5.20e-03
3.11e+00 nan 7.10e-03
3.34e+00 nan 9.46e-03
3.57e+00 nan 1.23e-02
3.80e+00 nan 1.58e-02
4.03e+00 1.55e-02 1.98e-02
4.32e+00 nan 2.60e-02
4.60e+00 nan 3.37e-02
4.89e+00 nan 4.32e-02
5.18e+00 nan 5.44e-02
5.47e+00 nan 6.77e-02
5.76e+00 nan 8.30e-02
6.04e+00 8.45e-02 1.006e-01
6.33e+00 nan 1.20e-01
6.62e+00 nan 1.44e-01
6.91e+00 nan 1.70e-01
7.20e+00 nan 2.01e-01
7.48e+00 nan 2.35e-01
7.77e+00 nan 2.74e-01
8.06e+00 2.58e-01 3.18e-01
8.64e+00 nan 4.19e-01
9.21e+00 nan 5.43e-01
9.79e+00 nan 6.92e-01
1.03e+01 nan 8.70e-01
1.09e+01 nan 1.07e+00
1.15e+01 nan 1.32e+00
1.20e+01 1.41e+00 1.60e+00


==> figures/Error_var_N64.tex <==
5.95e-01 1.23e-04 1.37e-04
6.52e-01 nan 1.98e-04
7.08e-01 nan 2.78e-04
7.65e-01 nan 3.80e-04
8.22e-01 nan 5.07e-04
8.78e-01 nan 6.61e-04
9.35e-01 nan 8.46e-04
9.92e-01 9.73e-04 1.06e-03
1.06e+00 nan 1.39e-03
1.13e+00 nan 1.80e-03
1.20e+00 nan 2.31e-03
1.27e+00 nan 2.91e-03
1.34e+00 nan 3.62e-03
1.41e+00 nan 4.45e-03
1.48e+00 4.84e-03 5.38e-03
1.55e+00 nan 6.46e-03
1.63e+00 nan 7.71e-03
1.70e+00 nan 9.14e-03
1.77e+00 nan 1.07e-02
1.84e+00 nan 1.26e-02
1.91e+00 nan 1.47e-02
1.98e+00 1.57e-02 1.70e-02
2.12e+00 nan 2.24e-02
2.26e+00 nan 2.91e-02
2.40e+00 nan 3.71e-02
2.55e+00 nan 4.66e-02
2.69e+00 nan 5.78e-02
2.83e+00 nan 7.09e-02
2.97e+00 8.12e-02 8.62e-02


==> figures/SE_VS_NewStyletau.tex <==
0.005000 5.056133 6.919579 7.113008 7.657857
0.010000 5.603976 6.947566 7.113008 7.657857
0.050000 7.027040 7.089215 7.113008 7.657857
0.100000 7.357293 7.061659 7.113008 7.657857
0.150000 7.489803 6.989555 7.113008 7.657857
0.200000 7.556089 6.944577 7.113008 7.657857
0.250000 7.560234 6.926046 7.113008 7.657857
0.300000 7.584667 6.912905 7.113008 7.657857


==> figures/SE_VS_Variance.tex <==
0.0001 10.1636555300254 10.1636673627025
0.306220408163265 10.1182923480564 10.1636673627025
0.612340816326531 10.072757462478 10.1636673627025
0.918461224489796 10.0376744903268 10.1636673627025
1.22458163265306 10.0038969116209 10.1636673627025
1.53070204081633 9.96042743311912 10.1636673627025
1.83682244897959 9.92587428381305 10.1636673627025
2.14294285714286 9.89669698224244 10.1636673627025
2.44906326530612 9.87255752124207 10.1636673627025
2.75518367346939 9.8422421494415 10.1636673627025
3.06130408163265 9.80931641383342 10.1636673627025
3.36742448979592 9.77449910994305 10.1636673627025
3.67354489795918 9.75198689269071 10.1636673627025
3.97966530612245 9.7464318709622 10.1636673627025
4.28578571428571 9.71459213477995 10.1636673627025
4.59190612244898 9.69168426715137 10.1636673627025
4.89802653061225 9.66881785289647 10.1636673627025
5.20414693877551 9.64593676226503 10.1636673627025
5.51026734693878 9.6105462611619 10.1636673627025
5.81638775510204 9.60417857485928 10.1636673627025
6.12250816326531 9.58668727457393 10.1636673627025
6.42862857142857 9.55969155482226 10.1636673627025
6.73474897959184 9.54426129998877 10.1636673627025
7.0408693877551 9.53594303066355 10.1636673627025
7.34698979591837 9.50008643534639 10.1636673627025
7.65311020408163 9.48790855849239 10.1636673627025
7.9592306122449 9.46285182909512 10.1636673627025
8.26535102040816 9.44268734330723 10.1636673627025
8.57147142857143 9.42396022806168 10.1636673627025
8.87759183673469 9.40175429363467 10.1636673627025
9.18371224489796 9.39545322957603 10.1636673627025
9.48983265306122 9.39515061897467 10.1636673627025
9.79595306122449 9.35831043856413 10.1636673627025
10.1020734693878 9.34211245297794 10.1636673627025
10.408193877551 9.32126919328523 10.1636673627025
10.7143142857143 9.33156013345342 10.1636673627025
11.0204346938776 9.30394214311237 10.1636673627025
11.3265551020408 9.28632634441549 10.1636673627025
11.6326755102041 9.30991377885038 10.1636673627025
11.9387959183673 9.26578794657152 10.1636673627025
12.2449163265306 9.26945651790575 10.1636673627025
12.5510367346939 9.2265954290093 10.1636673627025
12.8571571428571 9.21686350282789 10.1636673627025
13.1632775510204 9.20166628852809 10.1636673627025
13.4693979591837 9.19050852973754 10.1636673627025
13.7755183673469 9.18117109014336 10.1636673627025
14.0816387755102 9.16903965652951 10.1636673627025
14.3877591836735 9.16727337082426 10.1636673627025
14.6938795918367 9.158554224247 10.1636673627025
15.0 9.12308001127046 10.1636673627025


==> figures/SE_vs_Frequency_new.tex <==
10.0 17.377366720243840   15.979345193838000 13.135143555911425 13.900086297284568  15.905217669673630
20.0 15.362560740456763   14.212189906320631 12.170452499166617 12.285902066701063  14.182609023723778
30.0 14.178783351491795   13.150541111483653 11.583786869144200 11.335304415679948  13.136605223445082
40.0 13.335791026034768   12.390065480456280 11.333108494544044 10.657705609300270  12.383464280205505
50.0 12.679933104244796   11.797421592016416 11.272459302827533 10.125903555257520  11.793989548496112
60.0 12.142757862083307   11.314216285751270 11.173359566127303 9.691421912071120   11.316967060194393
70.0 11.687740874423360   10.905514065917556 10.834963169532404 9.327104876620010   10.903320528724302
80.0 11.293071222838353   10.551387981153818 10.499512908129644 8.997859259710240   10.544360931984546
90.0 10.944672216795425   10.241477321346910 10.117799689488663 8.718878064569004   10.226964372004806
100.0 10.632924938246372  9.962799653903957  9.839345574531380  8.455400239867210   9.948275104244571


==> figures/SE_vs_SNR_new.tex <==
10	2.87134301433954	2.61125874940118	2.5806505588074     2.350988531881764  2.609066262326155
12	3.63159957975187	3.31747467880476	3.26082711122316    2.882155278439049  3.312558112552793
14	4.4938148455785	4.12071981632395	4.04330417065638        3.507304186600108  4.114857595361387
16	5.45435951609528	5.01994123322604	4.91426084027804    4.253108201390649  5.011781004585681
18	6.50483823507947	6.0104370309192	5.84757790134472        5.092317633921049  5.996442933703457
20	7.63207765336568	7.08209648335968	6.93408306619672    6.001391101795271  7.066281502642859
22	8.82030115338407	8.22006156257028	8.02373733407542    6.977543895610245  8.199180291236102
24	10.0539793191025	9.40720438302396	9.18998908929335    7.987909838557670  9.389056041433749
26	11.3198515412662	10.6266778927748	10.4938926271609    9.011129794188381  10.611507831895045
28	12.6076794679352	11.863373518764	11.7986417535537        10.044040773820580  11.860402865623930
30	13.9100882021057	13.104206032011	12.709662076934         11.096936669540971  13.095721997306422
32	15.2220074704095	14.3376856052377	13.1830592225883    12.152228667200000  14.307251734089290
34	16.5400568678957	15.5532212353026	13.4534264446856    13.208650986932518  15.495088645995910
36	17.8620271363675	16.7404074776699	13.8560090521695    14.268548650605325  16.637272625241692
38	19.1864928075427	17.8883921253788	14.3828031092295    15.329420601728405  17.723726644389128
40	20.5125416314914	18.9853822308229	14.8476364473963    16.393416733425628  18.735562969234074


==> figures/gamma_dist_df_over_10.tex <==
16.18892 2.5680429851072815e-05
16.18895 2.6474854043232996e-05
16.18897 2.7292160768298385e-05
16.18899 2.813295348252258e-05
16.18901 2.8997849814468724e-05
16.18904 2.9887481847122502e-05
16.18906 3.080249640188572e-05
16.18908 3.1743555328956225e-05
16.1891 3.27113357999874e-05
16.18913 3.370653060560936e-05
16.18915 3.472984845789172e-05
16.18917 3.578201429541944e-05
16.18919 3.686376959378773e-05
16.18922 3.797587267971113e-05
16.18924 3.9119099049986674e-05
16.18926 4.029424169325795e-05
16.18928 4.1502111417783545e-05
16.18931 4.274353718262848e-05
16.18933 4.401936643200225e-05
16.18935 4.53304654363155e-05
16.18937 4.667771963485323e-05
16.1894 4.806203398434739e-05
16.18942 4.948433331113145e-05
16.18944 5.094556266760789e-05
16.18946 5.244668769291185e-05
16.18949 5.398869497762851e-05
16.18951 5.557259243346636e-05
16.18953 5.719940966498615e-05
16.18955 5.8870198348764676e-05
16.18958 6.058603261349434e-05
16.1896 6.234800942544238e-05
16.18962 6.415724897950398e-05
16.18964 6.601489509059756e-05
16.18967 6.79221155935477e-05
16.18969 6.98801027428342e-05
16.18971 7.189007361971498e-05
16.18973 7.395327053984e-05
16.18976 7.607096146800647e-05
16.18978 7.824444043531499e-05
16.1898 8.04750279581962e-05
16.18982 8.276407146570684e-05
16.18985 8.511294572475543e-05
16.18987 8.752305327476903e-05
16.18989 8.999582486070794e-05
16.18991 9.253271987390082e-05
16.18994 9.513522679198203e-05
16.18996 9.78048636265465e-05
16.18998 0.00010054317837092647
16.19 0.00010335174945216867
16.19003 0.0001062321861873342
16.19005 0.00010918612923899736
16.19007 0.00011221525107967575
16.19009 0.00011532125645331856
16.19012 0.0001185058828418469
16.19014 0.00012177090093681924
16.19016 0.0001251181151086167
16.19018 0.00012854936388200612
16.19021 0.00013206652041214078
16.19023 0.0001356714929648198
16.19025 0.00013936622539435572
16.19027 0.00014315269762904106
16.1903 0.00014703292615589531
16.19032 0.0001510089645037566
16.19034 0.00015508290373571283
16.19036 0.00015925687293481597
16.19039 0.00016353303969630302
16.19041 0.0001679136106193413
16.19043 0.00017240083179783936
16.19046 0.0001769969893176319
16.19048 0.00018170440974648312
16.1905 0.00018652546063252384
16.19052 0.00019146255099436227
16.19055 0.000196518131822165
16.19057 0.00020169469656643077
16.19059 0.0002069947816368091
16.19061 0.00021242096689650213
16.19064 0.00021797587615133264
16.19066 0.00022366217764886165
16.19068 0.00022948258456457042
16.1907 0.00023543985549706744
16.19073 0.00024153679495165595
16.19075 0.00024777625383252136
16.19077 0.0002541611299255835
16.19079 0.00026069436838159054
16.19082 0.00026737896219963304
16.19084 0.00027421795269914055
16.19086 0.000281214430002911
16.19088 0.00028837153350358435
16.19091 0.0002956924523320881
16.19093 0.00030318042582810916
16.19095 0.0003108387439950777
16.19097 0.000318670747960025
16.191 0.0003266798304246349
16.19102 0.0003348694361161964
16.19104 0.0003432430622233265
16.19106 0.00035180425883916185
16.19109 0.0003605566293930769
16.19111 0.00036950383106888724
16.19113 0.0003786495752351338
16.19115 0.0003879976278457752
16.19118 0.0003975518098573955
16.1912 0.0004073159976201016
16.19122 0.00041729412326826194
16.19124 0.0004274901751110894
16.19127 0.00043790819799839213
16.19129 0.0004485522936954257
16.19131 0.00045942662122973896
16.19133 0.00047053539725271776
16.19136 0.0004818828963645122
16.19138 0.0004934734514516539
16.1914 0.0005053114540055581
16.19142 0.0005174013544200882
16.19145 0.0005297476623018056
16.19147 0.000542354946743919
16.19149 0.0005552278366043589
16.19151 0.0005683710207656019
16.19154 0.0005817892483828968
16.19156 0.0005954873291194447
16.19158 0.0006094701333670113
16.1916 0.0006237425924598042
16.19163 0.0006383096988551787
16.19165 0.0006531765063294929
16.19167 0.0006683481301289823
16.19169 0.0006838297471244623
16.19172 0.0006996265959429028
16.19174 0.0007157439770839668
16.19176 0.0007321872530198192
16.19178 0.0007489618482764165
16.19181 0.0007660732495057404
16.19183 0.0007835270055173381
16.19185 0.0008013287273271269
16.19187 0.0008194840881530277
16.1919 0.000837998823405195
16.19192 0.0008568787306724732
16.19194 0.0008761296696499114
16.19196 0.0008957575620926476
16.19199 0.0009157683917059784
16.19201 0.0009361682040495823
16.19203 0.0009569631063849446
16.19205 0.0009781592675358385
16.19208 0.0009997629177007012
16.1921 0.0010217803482500975
16.19212 0.0010442179115099897
16.19214 0.0010670820204911255
16.19217 0.0010903791486407304
16.19219 0.001114115829524165
16.19221 0.0011382986564994816
16.19224 0.001162934282384802
16.19226 0.0011880294190613145
16.19228 0.0012135908370796374
16.1923 0.001239625365224872
16.19233 0.001266139890069333
16.19235 0.0012931413554643733
16.19237 0.0013206367620454823
16.19239 0.0013486331666896015
16.19242 0.0013771376819192017
16.19244 0.0014061574753330133
16.19246 0.0014356997689480534
16.19248 0.0014657718385490352
16.19251 0.0014963810129953693
16.19253 0.0015275346734839254
16.19255 0.0015592402528189695
16.19257 0.0015915052345958378
16.1926 0.0016243371524073957
16.19262 0.0016577435889587096
16.19264 0.0016917321752198317
16.19266 0.0017263105894792905
16.19269 0.0017614865563906547
16.19271 0.0017972678460152468
16.19273 0.001833662272756817
16.19275 0.0018706776943506122
16.19278 0.0019083220107364372
16.1928 0.0019466031629637127
16.19282 0.001985529131995228
16.19284 0.002025107937541604
16.19287 0.0020653476368120596
16.19289 0.002106256323244382
16.19291 0.002147842125215863
16.19293 0.002190113204662064
16.19296 0.0022330777557452966
16.19298 0.0022767440034023446
16.193 0.002321120201888631
16.19302 0.0023662146333188723
16.19305 0.0024120356060998217
16.19307 0.002458591453380205
16.19309 0.0025058905314364
16.19311 0.0025539412180475203
16.19314 0.002602751910772187
16.19316 0.0026523310252624228
16.19318 0.0027026869935041988
16.1932 0.0027538282619761667
16.19323 0.0028057632898708306
16.19325 0.0028585005471713043
16.19327 0.0029120485127571037
16.19329 0.0029664156724410317
16.19332 0.003021610516998965
16.19334 0.0030776415400921454
16.19336 0.0031345172362374826
16.19338 0.0031922460986992546
16.19341 0.0032508366172927673
16.19343 0.0033102972762704187
16.19345 0.003370636552018241
16.19347 0.003431862910867059
16.1935 0.00349398480674123
16.19352 0.0035570106788181443
16.19354 0.0036209489491982297
16.19356 0.003685808020432382
16.19359 0.0037515962731231936
16.19361 0.003818322063370167
16.19363 0.0038859937203263016
16.19365 0.003954619543551834
16.19368 0.0040242078004711105
16.1937 0.004094766723738899
16.19372 0.004166304508510973
16.19374 0.004238829309821132
16.19377 0.004312349239775602
16.19379 0.004386872364808007
16.19381 0.00446240670286478
16.19383 0.004538960220563038
16.19386 0.004616540830315511
16.19388 0.00469515638741636
16.1939 0.004774814687134876
16.19392 0.0048555234616716346
16.19395 0.004937290377250198
16.19397 0.005020123031018692
16.19399 0.0051040289479872
16.19402 0.005189015578000456
16.19404 0.005275090292549767
16.19406 0.005362260381661772
16.19408 0.005450533050711332
16.19411 0.00553991541725977
16.19413 0.005630414507756384
16.19415 0.005722037254356406
16.19417 0.005814790491650031
16.1942 0.005908680953289644
16.19422 0.006003715268789231
16.19424 0.00609989996006044
16.19426 0.006197241438173103
16.19429 0.006295745999898004
16.19431 0.006395419824309414
16.19433 0.006496268969446669
16.19435 0.006598299368801576
16.19438 0.006701516827914942
16.1944 0.006805927020900355
16.19442 0.006911535487015771
16.19444 0.007018347627091247
16.19447 0.007126368700112379
16.19449 0.00723560381971666
16.19451 0.007346057950588331
16.19453 0.007457735905064973
16.19456 0.007570642339509199
16.19458 0.007684781750821979
16.1946 0.00780015847289716
16.19462 0.007916776673082571
16.19465 0.00803464034863995
16.19467 0.008153753323194915
16.19469 0.008274119243248413
16.19471 0.008395741574530486
16.19474 0.008518623598609505
16.19476 0.008642768409265214
16.19478 0.008768178908967791
16.1948 0.008894857805471704
16.19483 0.009022807608156902
16.19485 0.009152030624697266
16.19487 0.00928252895745549
16.19489 0.0094143045001278
16.19492 0.009547358934176114
16.19494 0.009681693725495974
16.19496 0.009817310121006484
16.19498 0.009954209145145415
16.19501 0.010092391596669987
16.19503 0.010231858045127246
16.19505 0.010372608827705904
16.19507 0.010514644045802008
16.1951 0.010657963561870041
16.19512 0.010802566996054867
16.19514 0.010948453723105581
16.19516 0.011095622869143215
16.19519 0.011244073308522121
16.19521 0.011393803660790661
16.19523 0.01154481228748997
16.19525 0.011697097289304985
16.19528 0.011850656502956221
16.1953 0.012005487498257963
16.19532 0.012161587575339066
16.19534 0.012318953761664584
16.19537 0.012477582809298747
16.19539 0.012637471192126675
16.19541 0.012798615103220761
16.19543 0.01296101045205868
16.19546 0.013124652862050487
16.19548 0.013289537668003292
16.1955 0.013455659913504153
16.19552 0.013623014348693513
16.19555 0.013791595427754802
16.19557 0.013961397306688089
16.19559 0.014132413841079612
16.19561 0.01430463858386492
16.19564 0.014478064783375415
16.19566 0.014652685381152187
16.19568 0.014828493010134319
16.1957 0.015005479992598669
16.19573 0.015183638338570652
16.19575 0.015362959743867897
16.19577 0.015543435588591045
16.1958 0.015725056935546735
16.19582 0.01590781452859757
16.19584 0.016091698791458536
16.19586 0.016276699826180865
16.19589 0.016462807412057672
16.19591 0.01665001100429134
16.19593 0.016838299733074345
16.19595 0.017027662402526223
16.19598 0.017218087489798112
16.196 0.017409563144349355
16.19602 0.01760207718706152
16.19604 0.017795617109846944
16.19607 0.017990170074968406
16.19609 0.018185722914614833
16.19611 0.018382262130723474
16.19613 0.018579773894591
16.19616 0.0187782440468302
16.19618 0.018977658097313402
16.1962 0.01917800122533533
16.19622 0.019379258279629278
16.19625 0.019581413778805117
16.19627 0.01978445191174429
16.19629 0.019988356537930754
16.19631 0.020193111188314197
16.19634 0.020398699065754155
16.19636 0.020605103046103204
16.19638 0.020812305678972538
16.1964 0.021020289188778678
16.19643 0.021229035476059626
16.19645 0.021438526118555786
16.19647 0.021648742372769744
16.19649 0.021859665175254683
16.19652 0.02207127514449159
16.19654 0.02228355258235261
16.19656 0.022496477476121216
16.19658 0.022710029500451735
16.19661 0.022924188019266115
16.19663 0.023138932088195393
16.19665 0.023354240456691478
16.19667 0.023570091570541702
16.1967 0.02378646357439343
16.19672 0.02400333431441356
16.19674 0.024220681341065677
16.19676 0.02443848191198618
16.19679 0.024656712995087104
16.19681 0.024875351271484974
16.19683 0.02509437313900236
16.19685 0.02531375471533052
16.19688 0.025533471841600923
16.1969 0.025753500085963936
16.19692 0.025973814747301607
16.19694 0.026194390859056817
16.19697 0.026415203193158824
16.19699 0.026636226264175212
16.19701 0.02685743433328196
16.19703 0.02707880141280988
16.19706 0.027300301270460285
16.19708 0.027521907433817838
16.1971 0.027743593195160777
16.19712 0.027965331615918194
16.19715 0.028187095531794153
16.19717 0.028408857557499664
16.19719 0.028630590092001067
16.19721 0.02885226532348568
16.19724 0.029073855234823573
16.19726 0.029295331608855227
16.19728 0.02951666603387597
16.1973 0.029737829909315526
16.19733 0.02995879445122222
16.19735 0.0301795306983094
16.19737 0.030400009517656687
16.19739 0.030620201610692673
16.19742 0.03084007751943919
16.19744 0.031059607632498643
16.19746 0.03127876219141039
16.19749 0.03149751129696813
16.19751 0.031715824915755024
16.19753 0.03193367288649052
16.19755 0.032151024926810816
16.19758 0.03236785063996624
16.1976 0.03258411952142023
16.19762 0.03279980096596217
16.19764 0.03301486427444466
16.19767 0.033229278660885826
16.19769 0.03344301325955412
16.19771 0.03365603713203478
16.19773 0.033868319274633074
16.19776 0.03407982862546934
16.19778 0.034290534072011866
16.1978 0.03450040445828223
16.19782 0.03470940859257868
16.19785 0.03491751525483388
16.19787 0.03512469320420444
16.19789 0.035330911186884716
16.19791 0.03553613794353715
16.19794 0.03574034221728875
16.19796 0.03594349276130572
16.19798 0.036145558346788065
16.198 0.036346507770644874
16.19803 0.03654630986356288
16.19805 0.036744933497854036
16.19807 0.036942347595419325
16.19809 0.0371385211358221
16.19812 0.03733342316412435
16.19814 0.03752702279915477
16.19816 0.03771928924140359
16.19818 0.03791019178109903
16.19821 0.03809969980644003
16.19823 0.03828778281153553
16.19825 0.038474410404591916
16.19827 0.03865955231599328
16.1983 0.03884317840649302
16.19832 0.03902525867517155
16.19834 0.03920576326768451
16.19836 0.03938466248436143
16.19839 0.039561926788147087
16.19841 0.03973752681288836
16.19843 0.03991143337123079
16.19845 0.0400836174627347
16.19848 0.04025405028186455
16.1985 0.04042270322605278
16.19852 0.04058954790352245
16.19854 0.040754556141347535
16.19857 0.04091769999334775
16.19859 0.04107895174781132
16.19861 0.04123828393551775
16.19863 0.0413956693372953
16.19866 0.04155108099194825
16.19868 0.04170449220379971
16.1987 0.04185587655031701
16.19872 0.042005207889792014
16.19875 0.042152460368708636
16.19877 0.04229760842931179
16.19879 0.04244062681683983
16.19881 0.042581490587016275
16.19884 0.04272017511310924
16.19886 0.042856656093215865
16.19888 0.04299090955734682
16.1989 0.0431229118743215
16.19893 0.04325263975884949
16.19895 0.04338007027824617
16.19897 0.0435051808592383
16.19899 0.043627949294611196
16.19902 0.04374835374977291
16.19904 0.04386637276922158
16.19906 0.04398198528290371
16.19908 0.04409517061252737
16.19911 0.044205908477617926
16.19913 0.04431417900170435
16.19915 0.04441996271816744
16.19917 0.04452324057607402
16.1992 0.044623993945971364
16.19922 0.044722204625398325
16.19924 0.04481785484440859
16.19927 0.044910927270911234
16.19929 0.045001405015942665
16.19931 0.045089271638696464
16.19933 0.04517451115157138
16.19936 0.045257108025015404
16.19938 0.04533704719217204
16.1994 0.045414314053562964
16.19942 0.0454888944814248
16.19945 0.04556077482411157
16.19947 0.045629941910194365
16.19949 0.04569638305248725
16.19951 0.045760086051975825
16.19954 0.04582103920149376
16.19956 0.045879231289336374
16.19958 0.04593465160268794
16.1996 0.04598728993093085
16.19963 0.04603713656873575
16.19965 0.04608418231908541
16.19967 0.04612841849609901
16.19969 0.0461698369276683
16.19972 0.04620842995802515
16.19974 0.04624419045006032
16.19976 0.04627711178754101
16.19978 0.04630718787714761
16.19981 0.046334413150353304
16.19983 0.046358782565142295
16.19985 0.04638029160756438
16.19987 0.04639893629313682
16.1999 0.046414713168056836
16.19992 0.046427619310289214
16.19994 0.04643765233045326
16.19996 0.04644481037256299
16.19999 0.046449092114606017
16.20001 0.0464504967689416
16.20003 0.04644902408254812
16.20005 0.04644467433709667
16.20008 0.04643744834885977
16.2001 0.04642734746846069
16.20012 0.04641437358044947
16.20014 0.04639852910271285
16.20017 0.046379816985737
16.20019 0.0463582407116709
16.20021 0.04633380429327183
16.20023 0.04630651227263474
16.20026 0.0462763697198089
16.20028 0.046243382231205235
16.2003 0.04620755592789272
16.20032 0.04616889745367943
16.20035 0.04612741397307203
16.20037 0.04608311316906437
16.20039 0.04603600324074676
16.20041 0.04598609290081954
16.20044 0.04593339137285238
16.20046 0.045877908388483275
16.20048 0.04581965418442673
16.2005 0.04575863949928306
16.20053 0.04569487557028669
16.20055 0.045628374129833636
16.20057 0.04555914740189428
16.20059 0.04548720809823955
16.20062 0.045412569414610034
16.20064 0.04533524502662992
16.20066 0.04525524908562778
16.20068 0.0451725962143882
16.20071 0.045087301502603344
16.20073 0.04499938050235745
16.20075 0.044908849223367055
16.20077 0.044815724128122604
16.2008 0.04472002212694012
16.20082 0.04462176057276544
16.20084 0.044520957256019594
16.20086 0.0444176303991502
16.20089 0.044311798651245474
16.20091 0.04420348108229662
16.20093 0.044092697177605875
16.20095 0.043979466831858806
16.20098 0.043863810343170245
16.201 0.0437457484071199
16.20102 0.043625302110449446
16.20105 0.04350249292490737
16.20107 0.043377342700773626
16.20109 0.04324987366049986
16.20111 0.04312010839203506
16.20114 0.042988069842213525
16.20116 0.04285378131000022
16.20118 0.04271726643959086
16.2012 0.042578549213607146
16.20123 0.04243765394592532
16.20125 0.04229460527469869
16.20127 0.04214942815519131
16.20129 0.04200214785242643
16.20132 0.04185278993399295
16.20134 0.04170138026260347
16.20136 0.04154794498867179
16.20138 0.04139251054273931
16.20141 0.04123510362803544
16.20143 0.04107575121273721
16.20145 0.04091448052228941
16.20147 0.040751319031811215
16.2015 0.04058629445811939
16.20152 0.04041943475212726
16.20154 0.04025076809077911
16.20156 0.040080322869290586
16.20159 0.03990812769321919
16.20161 0.03973421137037132
16.20163 0.03955860290296843
16.20165 0.0393813314794836
16.20168 0.03920242646677948
16.2017 0.03902191740182581
16.20172 0.03883983398384891
16.20174 0.038656206066093025
16.20177 0.038471063647720766
16.20179 0.03828443686586198
16.20181 0.03809635598728785
16.20183 0.03790685140047148
16.20186 0.03771595360740186
16.20188 0.037523693215496194
16.2019 0.037330100929504874
16.20192 0.037135207543427445
16.20195 0.03693904393245889
16.20197 0.036741641044853855
16.20199 0.03654302989407489
16.20201 0.03634324155054976
16.20204 0.03614230713386866
16.20206 0.03594025780474382
16.20208 0.035737124757100315
16.2021 0.03553293921018387
16.20213 0.03532773240070546
16.20215 0.03512153557504205
16.20217 0.03491437998137621
16.20219 0.03470629686215655
16.20222 0.03449731744617303
16.20224 0.034287472941097075
16.20226 0.0340767945259028
16.20228 0.03386531334316502
16.20231 0.03365306049185545
16.20233 0.03344006701966915
16.20235 0.03322636391589036
16.20237 0.033011982103932344
16.2024 0.03279695243431862
16.20242 0.032581305677357376
16.20244 0.032365072516155446
16.20246 0.03214828353961629
16.20249 0.03193096923542254
16.20251 0.031713159983386176
16.20253 0.03149488604842446
16.20255 0.03127617757405303
16.20258 0.031057064575781248
16.2026 0.030837576934427565
16.20262 0.030617744389869802
16.20264 0.030397596534609477
16.20267 0.030177162807555058
16.20269 0.02995647248776842
16.20271 0.029735554688582026
16.20274 0.029514438351460753
16.20276 0.029293152240126595
16.20278 0.02907172493496682
16.2028 0.028850184827097874
16.20283 0.028628560112993265
16.20285 0.028406878788917345
16.20287 0.028185168645555578
16.20289 0.027963457262842342
16.20292 0.027741772004616378
16.20294 0.027520140013773123
16.20296 0.02729858820713531
16.20298 0.02707714327084085
16.20301 0.02685583165535861
16.20303 0.026634679571060024
16.20305 0.02641371298371639
16.20307 0.026192957609924634
16.2031 0.025972438913107587
16.20312 0.02575218209907413
16.20314 0.02553221211219198
16.20316 0.025312553631269958
16.20319 0.025093231065941825
16.20321 0.024874268552779882
16.20323 0.024655689951800487
16.20325 0.024437518842994024
16.20328 0.02421977852288064
16.2033 0.024002492001474265
16.20332 0.02378568199890868
16.20334 0.02356937094261789
16.20337 0.02335358096445056
16.20339 0.023138333897740615
16.20341 0.02292365127483759
16.20343 0.02270955432448339
16.20346 0.022496063969432586
16.20348 0.022283200824063775
16.2035 0.02207098519237566
16.20352 0.021859437065760077
16.20355 0.021648576121052615
16.20357 0.021438421718874195
16.20359 0.021228992901664634
16.20361 0.021020308392271505
16.20364 0.02081238659237133
16.20366 0.02060524558112731
16.20368 0.02039890311383855
16.2037 0.020193376620960993
16.20373 0.019988683206911436
16.20375 0.019784839649139067
16.20377 0.01958186239747658
16.20379 0.0193797675731747
16.20382 0.019178570968572194
16.20384 0.0189782880463481
16.20386 0.018778933939303404
16.20388 0.018580523450078195
16.20391 0.018383071050825057
16.20393 0.018186590883318324
16.20395 0.017991096758818194
16.20397 0.017796602158397956
16.204 0.017603120232929856
16.20402 0.017410663803659413
16.20404 0.017219245362470718
16.20406 0.017028877072412445
16.20409 0.016839570768477443
16.20411 0.016651337958094065
16.20413 0.016464189822108614
16.20415 0.016278137215604623
16.20418 0.016093190668908
16.2042 0.015909360388664976
16.20422 0.01572665625900741
16.20424 0.015545087842819548
16.20427 0.015364664382997956
16.20429 0.015185394804037182
16.20431 0.015007287713319063
16.20433 0.014830351402844374
16.20436 0.014654593850890704
16.20438 0.014480022723616566
16.2044 0.014306645377020569
16.20442 0.014134468858753775
16.20445 0.013963499910106742
16.20447 0.013793744967967333
16.20449 0.013625210167061379
16.20452 0.013457901341989787
16.20454 0.01329182402946181
16.20456 0.013126983470729787
16.20458 0.012963384613739798
16.20461 0.012801032115771835
16.20463 0.012639930345713262
16.20465 0.012480083386732508
16.20467 0.012321495038870166
16.2047 0.012164168821566736
16.20472 0.012008107976495609
16.20474 0.011853315470247495
16.20476 0.011699793997156949
16.20479 0.011547545982086415
16.20481 0.011396573583448324
16.20483 0.011246878696028187
16.20485 0.011098462953967495
16.20488 0.010951327733910202
16.2049 0.010805474157890585
16.20492 0.010660903096569111
16.20494 0.01051761517230613
16.20497 0.010375610762344428
16.20499 0.010234890002012144
16.20501 0.01009545278795708
16.20503 0.00995729878142186
16.20506 0.009820427411478308
16.20508 0.009684837878472016
16.2051 0.009550529157205018
16.20512 0.00941750000041665
16.20515 0.009285748942169823
16.20517 0.009155274301149046
16.20519 0.009026074184252046
16.20521 0.008898146489869637
16.20524 0.008771488911475294
16.20526 0.008646098940991463
16.20528 0.008521973872391902
16.2053 0.008399110805103548
16.20533 0.008277506647514829
16.20535 0.00815715812059251
16.20537 0.008038061761251086
16.20539 0.007920213926041149
16.20542 0.007803610794531056
16.20544 0.007688248372959603
16.20546 0.007574122497673926
16.20548 0.0074612288387706305
16.20551 0.007349562903533961
16.20553 0.0072391200400151725
16.20555 0.007129895440559757
16.20557 0.007021884145284509
16.2056 0.006915081045693562
16.20562 0.0068094808880606785
16.20564 0.006705078277019658
16.20566 0.006601867679053053
16.20569 0.006499843425893652
16.20571 0.00639899971807841
16.20573 0.006299330628359074
16.20575 0.006200830105158753
16.20578 0.006103491975955469
16.2058 0.006007309950772104
16.20582 0.005912277625493231
16.20584 0.0058183884852390354
16.20587 0.005725635907797082
16.20589 0.005634013166845427
16.20591 0.005543513435350597
16.20593 0.005454129788818553
16.20596 0.005365855208562288
16.20598 0.005278682584981941
16.206 0.0051926047207104505
16.20602 0.005107614333887601
16.20605 0.005023704061255736
16.20607 0.004940866461385383
16.20609 0.004859094017683634
16.20611 0.004778379141583378
16.20614 0.004698714175530334
16.20616 0.004620091396011076
16.20618 0.004542503016615456
16.2062 0.004465941190910352
16.20623 0.00439039801545254
16.20625 0.004315865532627283
16.20627 0.004242335733587877
16.2063 0.004169800561030245
16.20632 0.004098251912028189
16.20634 0.004027681640803072
16.20636 0.003958081561430225
16.20639 0.0038894434506042885
16.20641 0.003821759050223599
16.20643 0.0037550200700787934
16.20645 0.0036892181904461447
16.20648 0.003624345064596292
16.2065 0.003560392321371505
16.20652 0.0034973515676430507
16.20654 0.0034352143907699488
16.20657 0.0033739723609838676
16.20659 0.0033136170338139604
16.20661 0.003254139952375663
16.20663 0.0031955326496693574
16.20666 0.003137786650888885
16.20668 0.0030808934755693755
16.2067 0.0030248446398474754
16.20672 0.0029696316585341403
16.20675 0.0029152460472680855
16.20677 0.002861679324581927
16.20679 0.0028089230138902805
16.20681 0.0027569686455289864
16.20684 0.002705807758662035
16.20686 0.002655431903245611
16.20688 0.0026058326418376423
16.2069 0.0025570015514959684
16.20693 0.002508930225532386
16.20695 0.0024616102752711344
16.20697 0.0024150333318075207
16.20699 0.0023691910476331
16.20702 0.002324075098321238
16.20704 0.0022796771841115454
16.20706 0.0022359890314798073
16.20708 0.0021930023946660133
16.20711 0.002150709057164677
16.20713 0.002109100833181019
16.20715 0.002068169569029013
16.20717 0.0020279071445473734
16.2072 0.001988305474392764
16.20722 0.0019493565093816727
16.20724 0.0019110522377412686
16.20726 0.0018733846863444171
16.20729 0.0018363459219052295
16.20731 0.0017999280521389174
16.20733 0.001764123226889094
16.20735 0.0017289236392021101
16.20738 0.0016943215264139224
16.2074 0.0016603091711285512
16.20742 0.001626878902233009
16.20744 0.0015940230958480432
16.20747 0.0015617341762185716
16.20749 0.0015300046166394226
16.20751 0.0014988269402664098
16.20753 0.0014681937209675697
16.20756 0.0014380975840839994
16.20758 0.0014085312072130449
16.2076 0.0013794873209065294
16.20762 0.001350958709375986
16.20765 0.0013229382111543014
16.20767 0.0012954187197156196
16.20769 0.001268393184102424
16.20771 0.0012418546094654073
16.20774 0.001215796057629468
16.20776 0.0011902106476073754
16.20778 0.0011650915560664408
16.2078 0.0011404320178082098
16.20783 0.0011162253261883131
16.20785 0.0010924648335241935
16.20787 0.001069143951462252
16.20789 0.0010462561513483444
16.20792 0.0010237949645349824
16.20794 0.0010017539826815977
16.20796 0.000980126858047786
16.20799 0.0009589073037178519
16.20801 0.0009380890938472904
16.20803 0.0009176660638563997
16.20805 0.0008976321106100106
16.20808 0.0008779811925826615
16.2081 0.0008587073299765697
16.20812 0.00083980460485253
16.20814 0.0008212671612051171
16.20817 0.0008030892050518572
16.20819 0.000785265004461353
16.20821 0.0007677888895984902
16.20823 0.0007506552527340678
16.20826 0.0007338585482212835
16.20828 0.0007173932924891834
16.2083 0.0007012540639751729
16.20832 0.0006854355030773808
16.20835 0.000669932312059351
16.20837 0.0006547392549656339
16.20839 0.000639851157493103
16.20841 0.000625262906865695
16.20844 0.0006109694516866186
16.20846 0.0005969658017693598
16.20848 0.0005832470279725731
16.2085 0.000569808261991
16.20853 0.0005566446961602879
16.20855 0.0005437515832359957
16.20857 0.0005311242361497764
16.20859 0.0005187580277732273
16.20862 0.0005066483906527728
16.20864 0.0004947908167398555
16.20866 0.00048318085710231647
16.20868 0.00047181412163904365
16.20871 0.00046068627876483405
16.20873 0.0004497930550937543
16.20875 0.0004391302351209664
16.20877 0.00042869366087272423
16.2088 0.0004184792315694578
16.20882 0.00040848290326515375
16.20884 0.0003987006884840315
16.20886 0.00038912865584291815
16.20889 0.00037976292967753647
16.20891 0.00037059968964548573
16.20893 0.0003616351703292626
16.20895 0.0003528656608393102
16.20898 0.0003442875043914519
16.209 0.00033589709790070126
16.20902 0.00032769089154625517
16.20904 0.0003196653883485111
16.20907 0.00031181714373301864
16.20909 0.00030414276508337776
16.20911 0.0002966389113022592
16.20913 0.0002893022923539615
16.20916 0.00028212966881637
16.20918 0.0002751178514120508
16.2092 0.00026826370055362024
16.20922 0.0002615641258703998
16.20925 0.00025501608573785605
16.20927 0.0002486165868091625
16.20929 0.00024236268353071899
16.20931 0.00023625147766866123
16.20934 0.00023028011782427624
16.20936 0.00022444579895048534
16.20938 0.00021874576186584933
16.2094 0.00021317729276685435
16.20943 0.00020773772273915508
16.20945 0.00020242442726484954
16.20947 0.00019723482573585823
16.20949 0.00019216638095530432
16.20952 0.00018721659864890224
16.20954 0.00018238302697130295
16.20956 0.00017766325600866834
16.20958 0.00017305491728891628
16.20961 0.0001685556832859383
16.20963 0.00016416326692691841
16.20965 0.00015987542109752523
16.20967 0.00015568993815317795
16.2097 0.00015160464942418064
16.20972 0.00014761742472522944
16.20974 0.0001437261718692334
16.20977 0.00013992883617407458
16.20979 0.00013622339998096308
16.20981 0.00013260788216434366
16.20983 0.00012908033765144313
16.20986 0.00012563885694034601
16.20988 0.00012228156561752243
16.2099 0.00011900662388293825
16.20992 0.00011581222607298133
16.20995 0.00011269660018769371
16.20997 0.00010965800741858716
16.20999 0.00010669474168283473
16.21001 0.0001038051291551863
16.21004 0.00010098752780503252
16.21006 9.824032693855688e-05
16.21008 9.556194673814326e-05
16.2101 9.295083781065865e-05
16.21013 9.040548073508573e-05
16.21015 8.79243856147222e-05
16.21017 8.550609163239036e-05
16.21019 8.314916660896836e-05
16.21022 8.085220656549902e-05
16.21024 7.861383528762088e-05
16.21026 7.643270389654265e-05
16.21028 7.430749041890275e-05
16.21031 7.223689936476134e-05
16.21033 7.021966130734475e-05
16.21035 6.825453246491485e-05
16.21037 6.634029429064209e-05
16.2104 6.447575306131713e-05
16.21042 6.265973947436084e-05
16.21044 6.089110824525465e-05
16.21046 5.916873771214373e-05
16.21049 5.749152944141291e-05
16.21051 5.5858407838699965e-05
16.21053 5.426831976526678e-05
16.21055 5.2720234155041646e-05
16.21058 5.121314163993058e-05
16.2106 4.974605417516872e-05
16.21062 4.8318004672293985e-05
16.21064 4.692804663351887e-05
16.21067 4.557525379280658e-05
16.21069 4.425871975864552e-05
16.21071 4.297755766278603e-05
16.21073 4.173089981256963e-05
16.21076 4.0517897346970396e-05
16.21078 3.933771989848298e-05
16.2108 3.8189555256678794e-05
16.21082 3.707260903840891e-05
16.21085 3.5986104361163765e-05
16.21087 3.492928151985943e-05
16.21089 3.390139766956839e-05
16.21091 3.2901726511063924e-05
16.21094 3.192955798118505e-05
16.21096 3.0984197946805316e-05
16.21098 3.0064967904170467e-05
16.211 2.917120468085984e-05
16.21103 2.8302260142645758e-05
16.21105 2.745750090517272e-05
16.21107 2.663630804799677e-05
16.21109 2.583807683452461e-05
16.21112 2.5062216434870743e-05
16.21114 2.4308149653131055e-05
16.21116 2.3575312658984996e-05
16.21118 2.2863154722368907e-05
16.21121 2.2171137953431527e-05
16.21123 2.149873704516989e-05
16.21125 2.0845439021278442e-05
16.21127 2.021074298637562e-05
16.2113 1.9594159881771263e-05
16.21132 1.8995212243710637e-05
16.21134 1.8413433966008394e-05
16.21136 1.7848370066934673e-05
16.21139 1.7299576458692953e-05
16.21141 1.6766619721881998e-05
16.21143 1.6249076882619496e-05


==> figures/gamma_dist_df_over_2.tex <==
74.51851 0.00018932094635429783
74.53348 0.00019465402363890807
74.54845 0.00020012343130564985
74.56342 0.0002057322353305224
74.57839 0.00021148355875576428
74.59336 0.0002173805824335419
74.60833 0.00022342654577101417
74.6233 0.00022962474747649912
74.63827 0.00023597854630643997
74.65324 0.00024249136181296593
74.66821 0.00024916667509170904
74.68318 0.0002560080295296749
74.69815 0.0002630190315528019
74.71312 0.0002702033513729004
74.72809 0.000277564723733812
74.74306 0.0002851069486562789
74.75803 0.00029283389218131206
74.773 0.0003007494871117655
74.78797 0.00030885773375167845
74.80294 0.00031716270064310263
74.81791 0.00032566852530010684
74.83288 0.0003343794149394675
74.84785 0.00034329964720786633
74.86282 0.00035243357090501264
74.87779 0.00036178560670251385
74.89276 0.0003713602478579496
74.90773 0.00038116206092380555
74.9227 0.00039119568645093244
74.93767 0.0004014658396859949
74.95264 0.00041197731126256277
74.96761 0.00042273496788543014
74.98258 0.00043374375300772047
74.99755 0.0004450086875002348
75.01252 0.0004565348703128101
75.02749 0.0004683274791269942
75.04246 0.00048039177099970575
75.05743 0.0004927330829974545
75.0724 0.0005053568328204434
75.08737 0.0005182685194163448
75.10234 0.0005314737235829499
75.11731 0.0005449781085595101
75.13227 0.0005587874206059955
75.14724 0.0005729074895698581
75.16221 0.0005873442294399071
75.17718 0.0006021036388865253
75.19215 0.0006171918017878494
75.20712 0.000632614887741377
75.22209 0.0006483791525604366
75.23706 0.0006644909387548308
75.25203 0.0006809566759953934
75.267 0.0006977828815615777
75.28197 0.0007149761607717247
75.29694 0.0007325432073952972
75.31191 0.0007504908040466288
75.32688 0.0007688258225595388
75.34185 0.000787555224342103
75.35682 0.0008066860607112776
75.37179 0.0008262254732064613
75.38676 0.0008461806938815392
75.40173 0.0008665590455749161
75.4167 0.0008873679421566582
75.43167 0.0009086148887523032
75.44664 0.0009303074819427271
75.46161 0.0009524534099394063
75.47658 0.0009750604527344048
75.49155 0.000998136482224443
75.50652 0.0010216894623086472
75.52149 0.0010457274489589956
75.53646 0.0010702585902630326
75.55143 0.001095291126438316
75.5664 0.0011208333898175826
75.58137 0.0011468938048044385
75.59634 0.0011734808877986646
75.61131 0.0012006032470905212
75.62628 0.0012282695827233916
75.64125 0.0012564886863243678
75.65622 0.0012852694409017714
75.67119 0.00131462082060915
75.68616 0.0013445518904751917
75.70113 0.0013750718060988197
75.7161 0.0014061898133087749
75.73107 0.0014379152477870859
75.74604 0.0014702575346560128
75.76101 0.0015032261880274763
75.77598 0.0015368308105144864
75.79095 0.0015710810927042646
75.80592 0.0016059868125917658
75.82089 0.0016415578349736845
75.83586 0.0016778041108019691
75.85082 0.0017147356764962193
75.86579 0.0017523626532144393
75.88076 0.0017906952460817877
75.89573 0.0018297437433763084
75.9107 0.0018695185156712933
75.92567 0.001910030014933801
75.94064 0.0019512887735786643
75.95561 0.0019933054034773435
75.97058 0.0020360905949210945
75.98555 0.002079655115538271
76.00052 0.0021240098091647045
76.01549 0.002169165594666846
76.03046 0.002215133464717571
76.04543 0.0022619244845233076
76.0604 0.0023095497905028196
76.07537 0.0023580205889168464
76.09034 0.002407348154447902
76.10531 0.0024575438287302654
76.12028 0.002508619018829213
76.13525 0.0025605851956697545
76.15022 0.002613453892413728
76.16519 0.0026672367027850427
76.18016 0.0027219452793435434
76.19513 0.0027775913317057478
76.2101 0.002834186624712966
76.22507 0.002891742976546659
76.24004 0.0029502722567900552
76.25501 0.0030097863844360125
76.26998 0.003070297325841371
76.28495 0.0031318170926264532
76.29992 0.0031943577395207447
76.31489 0.003257931362153284
76.32986 0.003322550094788764
76.34483 0.003388226108008225
76.3598 0.0034549716063344933
76.37477 0.003522798825802737
76.38974 0.003591720031475186
76.40471 0.003661747514900315
76.41968 0.0037328935915167125
76.43465 0.003805170598001329
76.44962 0.0038785908895615524
76.46459 0.003953166837172438
76.47956 0.004028910824757766
76.49453 0.004105835246315509
76.5095 0.004183952502988471
76.52447 0.004263275000078661
76.53944 0.0043438151440073625
76.55441 0.00442558533921924
76.56938 0.00450859798503242
76.58434 0.00459286547243334
76.59931 0.004678400180817155
76.61428 0.00476521447467456
76.62925 0.004853320700224198
76.64422 0.004942731181991646
76.65919 0.005033458219335423
76.67416 0.005125514082920363
76.68913 0.005218911011137922
76.7041 0.005313661206475532
76.71907 0.005409776831833746
76.73404 0.005507270006792934
76.74901 0.00560615280382906
76.76398 0.005706437244480548
76.77895 0.00580813529546481
76.79392 0.005911258864746995
76.80889 0.0060158197975606845
76.82386 0.006121829872381101
76.83883 0.0062293007968517635
76.8538 0.006338244203665978
76.86877 0.006448671646402859
76.88374 0.006560594595319169
76.89871 0.006674024433098275
76.91368 0.00678897245055676
76.92865 0.006905449842308897
76.94362 0.007023467702391598
76.95859 0.007143037019849121
76.97356 0.0072641686742796864
76.98853 0.007386873431344172
77.0035 0.007511161938239505
77.01847 0.007637044719135433
77.03344 0.007764532170578312
77.04841 0.007893634556861795
77.06338 0.008024362005365526
77.07835 0.008156724501863371
77.09332 0.008290731885803275
77.10829 0.00842639384555857
77.12326 0.008563719913652817
77.13823 0.008702719461959958
77.1532 0.008843401696880875
77.16817 0.008985775654497239
77.18314 0.00912985019570454
77.19811 0.009275634001326732
77.21308 0.009423135567212323
77.22805 0.009572363199314225
77.24302 0.009723325008756093
77.25799 0.009876028906884361
77.27296 0.010030482600309908
77.28793 0.01018669358594016
77.30289 0.01034466914600279
77.31786 0.010504416343063167
77.33283 0.010665942015038458
77.3478 0.01082925277020799
77.36277 0.010994354982223686
77.37774 0.011161254785120228
77.39271 0.011329958068330589
77.40768 0.011500470471704117
77.42265 0.011672797380532013
77.43762 0.011846943920582408
77.45259 0.01202291495314515
77.46756 0.012200715070089138
77.48253 0.012380348588935584
77.4975 0.012561819547946301
77.51247 0.012745131701231902
77.52744 0.012930288513880752
77.54241 0.013117293157110247
77.55738 0.013306148503443653
77.57235 0.01349685712191328
77.58732 0.013689421273294457
77.60229 0.013883842905369483
77.61726 0.01408012364822557
77.63223 0.014278264809588827
77.6472 0.0144782673701967
77.66217 0.014680131979208871
77.67714 0.014883858949662892
77.69211 0.015089448253972635
77.70708 0.015296899519473979
77.72205 0.01550621202402082
77.73702 0.015717384691630476
77.75199 0.015930416088184216
77.76696 0.016145304417183523
77.78193 0.016362047515563694
77.7969 0.016580642849568627
77.81187 0.016801087510687478
77.82684 0.017023378211657683
77.84181 0.017247511282533847
77.85678 0.01747348266682635
77.87175 0.01770128791771219
77.88672 0.017930922194320197
77.90169 0.018162380258090728
77.91666 0.018395656469216214
77.93163 0.018630744783160937
77.9466 0.018867638747263587
77.96157 0.01910633149742669
77.97654 0.019346815754891906
77.99151 0.019589083823105112
78.00648 0.019833127584673895
78.02144 0.0200789384984192
78.03641 0.020326507596522266
78.05138 0.020575825481769613
78.06635 0.02082688232490018
78.08132 0.02107966786205322
78.09629 0.021334171392320838
78.11126 0.021590381775408157
78.12623 0.021848287429401893
78.1412 0.02210787632864816
78.15617 0.02236913600174524
78.17114 0.02263205352964913
78.18611 0.02289661554389551
78.20108 0.02316280822494204
78.21605 0.023430617300628953
78.23102 0.023700028044762112
78.24599 0.023971025275820613
78.26096 0.024243593355790103
78.27593 0.024517716189122678
78.2909 0.024793377221825647
78.30587 0.025070559440682934
78.32084 0.0253492453726067
78.33581 0.025629417084123488
78.35078 0.025911056180996254
78.36575 0.026194143807983558
78.38072 0.026478660648736232
78.39569 0.02676458692583357
78.41066 0.02705190240096251
78.42563 0.02734058637523744
78.4406 0.02763061768966364
78.45557 0.0279219747257476
78.47054 0.02821463540625069
78.48551 0.02850857719609175
78.50048 0.028803777103397956
78.51545 0.029100211680703852
78.53042 0.029397857026300444
78.54539 0.029696688785737033
78.56036 0.029996682153473283
78.57533 0.030297811874683743
78.5903 0.030600052247216975
78.60527 0.030903377123708366
78.62024 0.031207759913846934
78.63521 0.03151317358679675
78.65018 0.03181959067377625
78.66515 0.032126983270791436
78.68012 0.0324353230415253
78.69509 0.03274458122038653
78.71006 0.03305472861571154
78.72503 0.033365735613125995
78.74 0.033677572179063295
78.75496 0.03399020786443908
78.76993 0.03430361180848293
78.7849 0.0346177527427287
78.79987 0.03493259899515987
78.81484 0.03524811849451252
78.82981 0.03556427877473348
78.84478 0.03588104697959563
78.85975 0.03619838986746873
78.87472 0.036516273816243026
78.88969 0.03683466482841026
78.90466 0.03715352853629604
78.91963 0.03747283020744532
78.9346 0.037792534750162025
78.94957 0.03811260671919722
78.96454 0.03843301032158924
78.97951 0.03875370942265341
78.99448 0.03907466755211897
79.00945 0.03939584791041272
79.02442 0.03971721337509075
79.03939 0.04003872650741226
79.05436 0.0403603495590582
79.06933 0.040682044478990265
79.0843 0.041003772920451556
79.09927 0.04132549624810596
79.11424 0.0416471755453124
79.12921 0.04196877162153768
79.14418 0.04229024501990042
79.15915 0.04261155602484692
79.17412 0.04293266466995896
79.18909 0.043253530745886136
79.20406 0.04357411380840747
79.21903 0.04389437318661314
79.234 0.04421426799121109
79.24897 0.04453375712295053
79.26394 0.044852799281162495
79.27891 0.045171352972417
79.29388 0.045489376519290116
79.30885 0.045806828069240975
79.32382 0.046123665603597076
79.33879 0.04643984694664371
79.35376 0.04675532977481338
79.36873 0.047070071625977275
79.3837 0.047384029908830755
79.39867 0.04769716191237221
79.41364 0.0480094248154747
79.42861 0.048320775696543014
79.44358 0.04863117154325457
79.45855 0.04894056926238581
79.47351 0.049248925689712494
79.48848 0.04955619759998802
79.50345 0.049862341716991894
79.51842 0.05016731472364949
79.53339 0.050471073272214936
79.54836 0.05077357399451694
79.56333 0.05107477351226367
79.5783 0.05137462844740362
79.59327 0.05167309543253681
79.60824 0.05197013112137491
79.62321 0.05226569219924754
79.63818 0.05255973539364844
79.65315 0.052852217484818775
79.66812 0.05314309531636736
79.68309 0.05343232580591755
79.69806 0.05371986595578352
79.71303 0.05400567286366905
79.728 0.05428970373338469
79.74297 0.05457191588558039
79.75794 0.0548522667684914
79.77291 0.055130713968690424
79.78788 0.05540721522184387
79.80285 0.05568172842346936
79.81782 0.05595421163968924
79.83279 0.05622462311797516
79.84776 0.05649292129788374
79.86273 0.056759064821774965
79.8777 0.05702301254551124
79.89267 0.057284723549135455
79.90764 0.057544157147519884
79.92261 0.05780127290098468
79.93758 0.05805603062588192
79.95255 0.058308390405141367
79.96752 0.05855831259877237
79.98249 0.0588057578543192
79.99746 0.059050687117267846
80.01243 0.059293061641396125
80.0274 0.059532842999067165
80.04237 0.05976999309145966
80.05734 0.060004474158733265
80.07231 0.06023624879012419
80.08728 0.060465279933965846
80.10225 0.06069153090763442
80.11722 0.06091496540741138
80.13219 0.06113554751826188
80.14716 0.06135324172352532
80.16213 0.06156801291451234
80.1771 0.061779826400006725
80.19206 0.06198864791566827
80.20703 0.06219444363333151
80.222 0.062397180170197804
80.23697 0.06259682459791854
80.25194 0.06279334445156357
80.26691 0.06298670773847201
80.28188 0.06317688294698473
80.29685 0.06336383905505022
80.31182 0.06354754553870581
80.32679 0.06372797238042638
80.34176 0.06390509007734106
80.35673 0.06407886964931242
80.3717 0.06424928264687504
80.38667 0.06441630115903295
80.40164 0.06457989782090919
80.41661 0.06474004582124777
80.43158 0.06489671890976294
80.44655 0.0650498914043346
80.46152 0.06519953819804598
80.47649 0.0653456347660605
80.49146 0.06548815717233739
80.50643 0.06562708207618081
80.5214 0.0657623867386212
80.53637 0.06589404902862707
80.55134 0.06602204742914354
80.56631 0.06614636104295571
80.58128 0.0662669695983757
80.59625 0.06638385345474969
80.61122 0.06649699360778301
80.62619 0.06660637169468321
80.64116 0.06671196999911641
80.65613 0.06681377145597658
80.6711 0.06691175965596655
80.68607 0.06700591884998748
80.70104 0.06709623395333573
80.71601 0.06718269054970652
80.73098 0.06726527489500178
80.74595 0.067343973920941
80.76092 0.06741877523847384
80.77589 0.06748966714099391
80.79086 0.06755663860735184
80.80583 0.0676196793046659
80.8208 0.06767877959093149
80.83577 0.0677339305174261
80.85074 0.06778512383091005
80.86571 0.06783235197562287
80.88068 0.06787560809507323
80.89565 0.06791488603362329
80.91062 0.06795018033786573
80.92558 0.06798148625779443
80.94055 0.0680087997477669
80.95552 0.06803211746726005
80.97049 0.06805143678141716
80.98546 0.06806675576138829
81.00043 0.06807807318446157
81.0154 0.06808538853398825
81.03037 0.0680887019990992
81.04534 0.06808801447421498
81.06031 0.0680833275583488
81.07528 0.06807464355420377
81.09025 0.06806196546706339
81.10522 0.0680452970034781
81.12019 0.06802464256974683
81.13516 0.0680000072701949
81.15013 0.06797139690524955
81.1651 0.06793881796931374
81.18007 0.06790227764843867
81.19504 0.06786178381779782
81.21001 0.06781734503896139
81.22498 0.06776897055697478
81.23995 0.06771667029724049
81.25492 0.06766045486220636
81.26989 0.0676003355278608
81.28486 0.06753632424003653
81.29983 0.06746843361052583
81.3148 0.06739667691300674
81.32977 0.06732106807878417
81.34474 0.0672416216923472
81.35971 0.06715835298674303
81.37468 0.06707127783877245
81.38965 0.06698041276400614
81.40462 0.06688577491162566
81.41959 0.06678738205909095
81.43456 0.06668525260663648
81.44953 0.0665794055715981
81.4645 0.06646986058257401
81.47947 0.06635663787342144
81.49444 0.06623975827709158
81.50941 0.06611924321930641
81.52438 0.06599511471207842
81.53935 0.06586739534707726
81.55432 0.065736108288846
81.56929 0.06560127726786885
81.58426 0.06546292657349453
81.59923 0.06532108104671659
81.6142 0.06517576607281587
81.62917 0.06502700757386591
81.64413 0.06487483200110539
81.6591 0.06471926632718092
81.67407 0.06456033803826308
81.68904 0.06439807512603882
81.70401 0.06423250607958308
81.71898 0.0640636598771137
81.73395 0.06389156597763267
81.74892 0.06371625431245666
81.76389 0.06353775527664011
81.77886 0.06335609972029553
81.79383 0.06317131893981248
81.8088 0.06298344466898033
81.82377 0.06279250907001817
81.83874 0.0625985447245133
81.85371 0.062401584624274746
81.86868 0.062201662162104425
81.88365 0.06199881112248674
81.89862 0.061793065672205286
81.91359 0.061584460350885474
81.92856 0.061373030061470636
81.94353 0.06115881006063083
81.9585 0.060941835949112615
81.97347 0.06072214366203055
81.98844 0.060499769459104395
82.00341 0.060274749914846056
82.01838 0.06004712190870091
82.03335 0.0598169226151446
82.04832 0.05958418949374161
82.06329 0.059348960279168354
82.07826 0.05911127297120278
82.09323 0.058871165824686815
82.1082 0.05862867733946418
82.12317 0.0583838462502964
82.13814 0.05813671151676058
82.15311 0.05788731231313488
82.16808 0.05763568801827314
82.18305 0.05738187820547143
82.19802 0.05712592263233261
82.21299 0.05686786123063134
82.22796 0.05660773409618207
82.24293 0.05634558147871401
82.2579 0.056081443771758804
82.27287 0.0558153615025496
82.28784 0.055547375321939985
82.30281 0.05527752599434349
82.31778 0.05500585438769609
82.33275 0.05473240146344783
82.34772 0.0544572082665854
82.36269 0.05418031591568836
82.37765 0.05390176559302233
82.39262 0.053621598534674346
82.40759 0.053339856020731616
82.42256 0.053056579365505875
82.43753 0.05277180990780942
82.4525 0.05248558900128409
82.46747 0.05219795800478553
82.48244 0.05190895827282617
82.49741 0.05161863114608259
82.51238 0.051327017941964384
82.52735 0.05103415994525318
82.54232 0.05074009839881106
82.55729 0.05044487449436313
82.57226 0.0501485293633537
82.58723 0.04985110406788402
82.6022 0.04955263959172885
82.61717 0.049253176831437
82.63214 0.04895275658751869
82.64711 0.048651419555721866
82.66208 0.04834920631839704
82.67705 0.048046157335957795
82.69202 0.04774231293843657
82.70699 0.04743771331713588
82.72196 0.04713239851638252
82.73693 0.04682640842538172
82.7519 0.04651978277017513
82.76687 0.046212561105706304
82.78184 0.04590478280799277
82.79681 0.045596487066409105
82.81178 0.045287712876079494
82.82675 0.04497849903038639
82.84172 0.04466888411359231
82.85669 0.044358906493578196
82.87166 0.044048604314701194
82.88663 0.04373801549077215
82.9016 0.04342717769815258
82.91657 0.04311612836897625
82.93154 0.04280490468449344
82.94651 0.04249354356854141
82.96148 0.042182081681140376
82.97645 0.04187055541221656
82.99142 0.04155900087545644
83.00639 0.041247453902287
83.02136 0.040935950035989585
83.03633 0.040624524525944554
83.0513 0.04031321232200691
83.06627 0.04000204806901651
83.08124 0.039691066101443455
83.0962 0.03938030043816374
83.11117 0.03906978477737434
83.12614 0.0387595524916429
83.14111 0.038449636623091775
83.15608 0.03814006987872098
83.17105 0.037830884625866805
83.18602 0.03752211288779884
83.20099 0.037213786339453374
83.21596 0.03690593630330449
83.23093 0.03659859374537504
83.2459 0.0362917892713828
83.26087 0.03598555312302656
83.27584 0.03567991517441026
83.29081 0.035374904928603304
83.30578 0.03507055151434006
83.32075 0.03476688368285738
83.33572 0.03446392980486771
83.35069 0.03416171786767113
83.36566 0.033860275472401134
83.38063 0.03355962983141145
83.3956 0.033259807765794555
83.41057 0.032960835703035686
83.42554 0.03266273967480541
83.44051 0.03236554531488233
83.45548 0.03206927785721051
83.47045 0.03177396213409171
83.48542 0.03147962257450571
83.50039 0.03118628320256713
83.51536 0.03089396763610887
83.53033 0.0306026990853951
83.5453 0.030312500351967007
83.56027 0.030023393827611933
83.57524 0.029735401493460982
83.59021 0.02944854491921347
83.60518 0.029162845262484857
83.62015 0.028878323268277092
83.63512 0.0285949992685752
83.65009 0.02831289318206176
83.66506 0.028032024513951016
83.68003 0.02775241235594653
83.695 0.02747407538631071
83.70997 0.027197031870052568
83.72494 0.026921299659233077
83.73991 0.02664689619338037
83.75488 0.026373838500017257
83.76985 0.026102143195302838
83.78482 0.025831826484779667
83.79979 0.025562904164229402
83.81475 0.025295391620636546
83.82972 0.025029303833254784
83.84469 0.024764655374776064
83.85966 0.024501460412604287
83.87463 0.024239732710225653
83.8896 0.02397948562867748
83.90457 0.023720732128116734
83.91954 0.02346348476948006
83.93451 0.023207755716238124
83.94948 0.02295355673624324
83.96445 0.022700899203663326
83.97942 0.022449794101008454
83.99439 0.022200252021240256
84.00936 0.021952283169966304
84.02433 0.021705897367720228
84.0393 0.02146110405231959
84.05427 0.02121791228130425
84.06924 0.020976330734453184
84.08421 0.020736367716375964
84.09918 0.020498031159177085
84.11415 0.020261328625195675
84.12912 0.020026267309812305
84.14409 0.01979285404432431
84.15906 0.01956109529889068
84.17403 0.019330997185538386
84.189 0.019102565461232693
84.20397 0.018875805531009662
84.21894 0.018650722451166616
84.23391 0.01842732093250914
84.24888 0.018205605343657158
84.26385 0.017985579714399704
84.27882 0.01776724773910696
84.29379 0.017550612780187914
84.30876 0.01733567787159761
84.32373 0.017122445722392975
84.3387 0.016910918720330452
84.35367 0.016701098935506635
84.36864 0.01649298812404255
84.38361 0.016286587731804275
84.39858 0.016081898898161726
84.41355 0.01587892245978442
84.42852 0.015677658954469813
84.44349 0.015478108625003173
84.45846 0.015280271423050584
84.47343 0.015084147013078046
84.4884 0.014889734776297636
84.50337 0.01469703381464135
84.51834 0.014506042954756089
84.53331 0.014316760752020999
84.54827 0.014129185494586527
84.56324 0.01394331520743066
84.57821 0.013759147656431764
84.59318 0.013576680352459262
84.60815 0.013395910555475716
84.62312 0.013216835278651218
84.63809 0.013039451292490728
84.65306 0.0128637551289682
84.66803 0.012689743085668876
84.683 0.012517411229938822
84.69797 0.012346755403038014
84.71294 0.012177771224296119
84.72791 0.012010454095272457
84.74288 0.01184479920391279
84.75785 0.011680801528708639
84.77282 0.01151845584285152
84.78779 0.0113577567183842
84.80276 0.011198698530347561
84.81773 0.011041275460920307
84.8327 0.010885481503550128
84.84767 0.010731310467078316
84.86264 0.010578755979851901
84.87761 0.010427811493824322
84.89258 0.010278470288645987
84.90755 0.010130725475737963
84.92252 0.009984570002351758
84.93749 0.009839996655614386
84.95246 0.00969699806655452
84.96743 0.009555566714110241
84.9824 0.009415694929119455
84.99737 0.00927737489828789
85.01234 0.00914059866813635
85.02731 0.00900535814892653
85.04228 0.008871645118561576
85.05725 0.008739451226464925
85.07222 0.008608767997432041
85.08719 0.008479586835456231
85.10216 0.008351899027529178
85.11713 0.008225695747412089
85.1321 0.008100968059378657
85.14707 0.007977706921929508
85.16204 0.0078559031914758
85.17701 0.007735547625991543
85.19198 0.007616630888636144
85.20695 0.007499143551342985
85.22192 0.007383076098375324
85.23689 0.007268418929849976
85.25186 0.007155162365225373
85.26682 0.007043296646755229
85.28179 0.006932811942907593
85.29676 0.006823698351747272
85.31173 0.0067159459042815456
85.3267 0.006609544567770499
85.34167 0.006504484248998442
85.35664 0.006400754797507586
85.37161 0.006298346008794821
85.38658 0.006197247627468326
85.40155 0.006097449350365461
85.41652 0.005998940829631886
85.43149 0.005901711675760177
85.44646 0.005805751460588098
85.46143 0.005711049720257682
85.4764 0.005617595958132315
85.49137 0.005525379647673205
85.50634 0.005434390235275165
85.52131 0.005344617143060416
85.53628 0.005256049771630437
85.55125 0.005168677502777228
85.56622 0.005082489702151373
85.58119 0.0049974757218880835
85.59616 0.004913624903192083
85.61113 0.004830926578878587
85.6261 0.004749370075873117
85.64107 0.004668944717668135
85.65604 0.004589639826736798
85.67101 0.004511444726905266
85.68598 0.004434348745681289
85.70095 0.004358341216540189
85.71592 0.004283411481169246
85.73089 0.004209548891668385
85.74586 0.004136742812708706
85.76083 0.004064982623648862
85.7758 0.0039942577206086355
85.79077 0.003924557518500034
85.80574 0.003855871453017032
85.82071 0.0037881889825824113
85.83568 0.003721499590252638
85.85065 0.003655792785581804
85.86562 0.003591058106443044
85.88059 0.0035272851208087313
85.89556 0.0034644634284897507
85.91053 0.0034025826628333593
85.9255 0.003341632492379969
85.94047 0.0032816026224801917
85.95544 0.003222482796870229
85.97041 0.003164262799208325
85.98537 0.003106932454570514
86.00034 0.003050481630906871
86.01531 0.0029949002404588065
86.03028 0.0029401782411369206
86.04525 0.0028863056378599203
86.06022 0.002833272483855803
86.07519 0.002781068881924211
86.09016 0.0027296849856608962
86.10513 0.0026791110006455913
86.1201 0.0026293371855916387
86.13507 0.002580353853459231
86.15004 0.0025321513725326287
86.16501 0.0024847201674606844
86.17998 0.0024380507202616513
86.19495 0.0023921335712932448
86.20992 0.0023469593201871104
86.22489 0.002302518626748825
86.23986 0.0022588022118240378
86.25483 0.002215800858130468
86.2698 0.0021735054110564333
86.28477 0.002131906779426907
86.29974 0.0020909959362364803
86.31471 0.0020507639193501613
86.32968 0.002011201832172934
86.34465 0.0019723008442874734
86.35962 0.0019340521920610746
86.37459 0.0018964471792223521
86.38956 0.001859477177407672
86.40453 0.0018231336266778676
86.4195 0.0017874080360063005
86.43447 0.0017522919837374537
86.44944 0.0017177771180179773
86.46441 0.0016838551571993785
86.47938 0.0016505178902134167
86.49435 0.0016177571769207348
86.50932 0.001585564948432807
86.52429 0.0015539332074076741
86.53926 0.0015228540283205396
86.55423 0.0014923195577087305
86.5692 0.0014623220143919994
86.58417 0.0014328536896688912
86.59914 0.001403906947488896
86.61411 0.0013754742246013365
86.62908 0.001347548030681462
86.64405 0.001320120948433911
86.65902 0.0012931856336740144
86.67399 0.0012667348153878773
86.68896 0.001240761295770942
86.70393 0.001215257950245908
86.71889 0.0011902177274605327
86.73386 0.001165633649265449
86.74883 0.0011414988106724752
86.7638 0.0011178063797943132
86.77877 0.0010945495977652117
86.79374 0.00107172177864399
86.80871 0.001049316309299058
86.82368 0.0010273266492762073
86.83865 0.0010057463306497344
86.85362 0.0009845689578569718
86.86859 0.0009637882075167495
86.88356 0.0009433978282325453
86.89853 0.000923391640380148
86.9135 0.0009037635358805754
86.92847 0.0008845074779588236
86.94344 0.0008656175008883861
86.95841 0.0008470877097222305
86.97338 0.0008289122800107064
86.98835 0.0008110854575064984
87.00332 0.0007936015578571085
87.01829 0.0007764549662855185
87.03326 0.0007596401372589321
87.04823 0.0007431515941462405
87.0632 0.0007269839288647461
87.07817 0.0007111318015160813
87.09314 0.0006955899400119628
87.10811 0.0006803531396901986
87.12308 0.0006654162629210563
87.13805 0.0006507742387044181
87.15302 0.0006364220622583248
87.16799 0.0006223547945988109
87.18296 0.0006085675621115943
87.19793 0.0005950555561160998
87.2129 0.0005818140324218408
87.22787 0.0005688383108774971
87.24284 0.0005561237749133997
87.25781 0.000543665871077207
87.27278 0.0005314601085633294
87.28775 0.0005195020587365517
87.30272 0.0005077873546497498
87.31769 0.0004963116905564068
87.33266 0.0004850708214179204
87.34763 0.0004740605624060634
87.3626 0.00046327678840103677
87.37757 0.00045271543348509804
87.39254 0.0004423724904321875
87.40751 0.00043224401019391757
87.42248 0.000422326101381943
87.43744 0.0004126149297470967
87.45241 0.00040310671765561075
87.46738 0.0003937977435624284
87.48235 0.0003846843414821644
87.49732 0.00037576290045762293
87.51229 0.00036702986402634206
87.52726 0.00035848172968519726
87.54223 0.0003501150483535203
87.5572 0.0003419264238346706
87.57217 0.0003339125122764397
87.58714 0.00032607002163049495
87.60211 0.00031839571111097096
87.61708 0.0003108863906524213
87.63205 0.00030353892036746747
87.64702 0.0002963502100040501
87.66199 0.0002893172184027718
87.67696 0.0002824369529542685
87.69193 0.0002757064690568825
87.7069 0.0002691228695748405
87.72187 0.00026268330429702214
87.73684 0.00025638496939647056
87.75181 0.0002502251068909386
87.76678 0.0002442010041044316
87.78175 0.0002383099931299871
87.79672 0.00023254945029389936
87.81169 0.0002269167956213936
87.82666 0.0002214094923039141
87.84163 0.0002160250461682954
87.8566 0.00021076100514773956
87.87157 0.0002056149587548258
87.88654 0.0002005845375567233
87.90151 0.00019566741265258987
87.91648 0.00019086129515335528
87.93145 0.00018616393566400085
87.94642 0.00018157312376839005
87.96139 0.00017708668751675185
87.97636 0.0001727024929160026
87.99133 0.00016841844342286403
88.0063 0.00016423247943994255
88.02127 0.00016014257781489063
88.03624 0.00015614675134263895
88.05121 0.00015224304827083304
88.06618 0.00014842955180857285
88.08115 0.0001447043796384722
88.09612 0.00014106568343212036
88.11109 0.00013751164836908164
88.12606 0.00013404049265936012
88.14103 0.00013065046706954627
88.156 0.00012733985445257388
88.17096 0.00012410696928120214
88.18593 0.00012095015718528861
88.2009 0.00011786779449285748
88.21587 0.00011485828777502
88.23084 0.00011192007339484344
88.24581 0.00010905161706012451
88.26078 0.00010625141338015375
88.27575 0.00010351798542653287
88.29072 0.00010084988429800842
88.30569 9.824568868940148e-05
88.32066 9.570400446466924e-05
88.33563 9.322346423406736e-05
88.3506 9.080272693552511e-05
88.36557 8.844047742016612e-05
88.38054 8.613542604203917e-05
88.39551 8.388630825209867e-05
88.41048 8.169188419639031e-05
88.42545 7.955093831851217e-05
88.44042 7.746227896630886e-05
88.45539 7.54247380028822e-05
88.47036 7.343717042183383e-05
88.48533 7.149845396683586e-05
88.5003 6.960748875546465e-05
88.51527 6.776319690733224e-05
88.53024 6.596452217652433e-05
88.54521 6.421042958831895e-05
88.56018 6.249990508019039e-05
88.57515 6.083195514712339e-05
88.59012 5.920560649118613e-05
88.60509 5.7619905675379e-05
88.62006 5.607391878176919e-05
88.63503 5.456673107386119e-05
88.65 5.309744666321932e-05
88.66497 5.166518818033194e-05
88.67994 5.026909644968748e-05
88.69491 4.89083301690521e-05
88.70988 4.7582065592956244e-05
88.72485 4.628949622033609e-05
88.73982 4.5029832486331754e-05
88.75479 4.380230145823784e-05
88.76976 4.260614653555409e-05
88.78473 4.144062715413525e-05
88.7997 4.0305018494423035e-05
88.81467 3.91986111937214e-05
88.82964 3.8120711062496496e-05
88.84461 3.7070638804694156e-05
88.85958 3.604772974202221e-05
88.87455 3.505133354218503e-05
88.88951 3.4080813951056985e-05
88.90448 3.313554852874041e-05
88.91945 3.221492838949778e-05
88.93442 3.131835794553227e-05
88.94939 3.044525465456817e-05
88.96436 2.9595048771229992e-05
88.97933 2.876718310216197e-05
88.9943 2.796111276486996e-05
89.00927 2.7176304950264312e-05
89.02424 2.641223868885256e-05
89.03921 2.566840462055505e-05
89.05418 2.4944304768129147e-05
89.06915 2.4239452314141877e-05
89.08412 2.3553371381472358e-05
89.09909 2.288559681731691e-05
89.11406 2.2235673980645097e-05
89.12903 2.160315853308501e-05
89.144 2.098761623320458e-05
89.15897 2.0388622734141843e-05
89.17394 1.980576338456737e-05
89.18891 1.9238633032926738e-05
89.20388 1.8686835834934465e-05
89.21885 1.814998506429282e-05
89.23382 1.762770292658248e-05
89.24879 1.71196203763025e-05
89.26376 1.662537693702191e-05
89.27873 1.6144620524602147e-05
89.2937 1.567700727345721e-05
89.30867 1.522220136582066e-05
89.32364 1.4779874863974197e-05
89.33861 1.4349707545406099e-05
89.35358 1.3931386740869585e-05
89.36855 1.3524607175294144e-05
89.38352 1.3129070811520309e-05
89.39849 1.2744486696824603e-05
89.41346 1.2370570812191901e-05
89.42843 1.2007045924302628e-05
89.4434 1.1653641440204553e-05
89.45837 1.1310093264623709e-05
89.47334 1.097614365988451e-05


==> figures/gamma_hist_df_over_10.tex <==
16.18883 0.0001
16.18917 0.0002
16.1895 0.0
16.18983 0.0
16.19017 0.0002
16.1905 0.0003
16.19083 0.0003
16.19117 0.0005
16.1915 0.0002
16.19183 0.0011
16.19217 0.0006
16.1925 0.0014
16.19283 0.0023
16.19317 0.0023
16.1935 0.004
16.19383 0.0034
16.19417 0.0055
16.1945 0.0076
16.19483 0.0095
16.19517 0.012
16.1955 0.0126
16.19583 0.0169
16.19617 0.0185
16.1965 0.0211
16.19683 0.024
16.19717 0.0289
16.1975 0.0323
16.19783 0.0336
16.19817 0.0402
16.1985 0.0418
16.19883 0.0403
16.19917 0.0459
16.1995 0.0472
16.19983 0.0447
16.20017 0.0454
16.2005 0.0453
16.20083 0.0471
16.20117 0.0436
16.2015 0.0404
16.20183 0.0366
16.20217 0.0353
16.2025 0.0317
16.20283 0.0268
16.20317 0.0256
16.2035 0.0215
16.20383 0.0183
16.20417 0.0156
16.2045 0.0134
16.20483 0.0117
16.20517 0.0087
16.2055 0.008
16.20583 0.0067
16.20617 0.0059
16.2065 0.0033
16.20683 0.0024
16.20717 0.0022
16.2075 0.0011
16.20783 0.0014
16.20817 0.0012
16.2085 0.0001
16.20883 0.0005
16.20917 0.0002
16.2095 0.0002
16.20983 0.0
16.21017 0.0001
16.2105 0.0
16.21083 0.0
16.21117 0.0001
16.2115 0.0001


==> figures/gamma_hist_df_over_2.tex <==
73.83333 0.0001
74.16667 0.0
74.5 0.0
74.83333 0.0001
75.16667 0.0003
75.5 0.0005
75.83333 0.0013
76.16667 0.0024
76.5 0.0036
76.83333 0.005
77.16667 0.0085
77.5 0.0109
77.83333 0.0178
78.16667 0.0225
78.5 0.0308
78.83333 0.0419
79.16667 0.0416
79.5 0.0544
79.83333 0.0559
80.16667 0.0639
80.5 0.0711
80.83333 0.0647
81.16667 0.0679
81.5 0.0671
81.83333 0.0609
82.16667 0.0572
82.5 0.0488
82.83333 0.0416
83.16667 0.0341
83.5 0.0298
83.83333 0.0248
84.16667 0.0196
84.5 0.0117
84.83333 0.0121
85.16667 0.0088
85.5 0.0064
85.83333 0.0039
86.16667 0.0022
86.5 0.002
86.83333 0.0014
87.16667 0.0006
87.5 0.0004
87.83333 0.0002
88.16667 0.0006
88.5 0.0003
88.83333 0.0001
89.16667 0.0001
89.5 0.0
89.83333 0.0
90.16667 0.0
90.5 0.0
90.83333 0.0
91.16667 0.0001

